A Conflict-Aware Optimal Goal Assignment Algorithm for Multi-Robot Systems

The fundamental goal assignment problem for a multi-robot application aims to assign a unique goal to each robot while ensuring collision-free paths, minimizing the total movement cost. A plausible algorithmic solution to this NP-hard problem involves an iterative process that integrates a task planner to compute the goal assignment while ignoring the collision possibilities among the robots and a multi-agent path-finding algorithm to find the collision-free trajectories for a given assignment. This procedure involves a method for computing the next best assignment given the current best assignment. A naive way of computing the next best assignment, as done in the state-of-the-art solutions, becomes a roadblock to achieving scalability in solving the overall problem. To obviate this bottleneck, we propose an efficient conflict-guided method to compute the next best assignment. Additionally, we introduce two more optimizations to the algorithm -- first for avoiding the unconstrained path computations between robot-goal pairs wherever possible, and the second to prevent duplicate constrained path computations for multiple robot-goal pairs. We extensively evaluate our algorithm for up to a hundred robots on several benchmark workspaces. The results demonstrate that the proposed algorithm achieves nearly an order of magnitude speedup over the state-of-the-art algorithm, showcasing its efficacy in real-world scenarios.

==> plots_scatter.tex <==
% SCATTER PLOTS

\begin{figure}[!ht]
    % SYDNEY
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        % \centering
        \includegraphics[scale=0.27]{plots/scatter_syd_50R.pdf}
        \includegraphics[scale=0.27]{plots/scatter_syd_100R.pdf}
        % \includegraphics[scale=0.18]{plots/s1.pdf}
        \caption{Sydney ($256 \times 256$)}
        \label{fig:scatter-sydney}
    \end{subfigure}
    
    % WAREHOUSE
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.27]{plots/scatter_ware_50R.pdf}
        \includegraphics[scale=0.27]{plots/scatter_ware_100R.pdf}
        % \includegraphics[scale=0.18]{plots/s1.pdf}
        \caption{Warehouse ($123 \times 321$)}
        \label{fig:scatter-warehouse}
    \end{subfigure}
    
    % DEN
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.27]{plots/scatter_den_50R.pdf}
        \includegraphics[scale=0.27]{plots/scatter_den_100R.pdf}
        % \includegraphics[scale=0.18]{plots/s1.pdf}
        \caption{Den ($257 \times 256$)}
        \label{fig:scatter-den}
    \end{subfigure}
    
    % RANDOM_200 
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.27]{plots/scatter_random_50R.pdf}
        \includegraphics[scale=0.27]{plots/scatter_random_100R.pdf}
        % \includegraphics[scale=0.18]{plots/s1.pdf}
        \caption{Random ($200 \times 200$)}
        \label{fig:scatter-random}
    \end{subfigure}
    
    
    

    \caption{Scatter Plots for Different Workspace 
    % \\ (\textit{X-axis:} $\log{(\text{Runtime(\si{\second})})}$ of (p0h0c0), \textit{Y-axis:} $\log{(\text{Runtime(\si{\second})})}$ 
    \\ \hspace*{1.3cm} (Left: $R = 50$, Right: $R = 100$)  
    }
    \label{fig:scatter_plots}
\end{figure}



==> plots_scatter_a2.tex <==
% SCATTER PLOTS

\begin{figure}[!ht]
    
    % RANDOM_200 
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.24]{plots_a2/scatter_random_50R_a2.pdf}
        \includegraphics[scale=0.24]{plots_a2/scatter_random_100R_a2.pdf}
        % \includegraphics[scale=0.18]{plots/s1.pdf}
        \caption{Random ($200 \times 200$)}
        \label{fig:scatter-random}
    \end{subfigure}
    
    
    % WAREHOUSE
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.24]{plots_a2/scatter_ware_50R_a2.pdf}
        \includegraphics[scale=0.24]{plots_a2/scatter_ware_100R_a2.pdf}
        % \includegraphics[scale=0.18]{plots/s1.pdf}
        \caption{Warehouse ($123 \times 321$)}
        \label{fig:scatter-warehouse}
    \end{subfigure}
    
    
    % SYDNEY
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        % \centering
        \includegraphics[scale=0.24]{plots_a2/scatter_syd_50R_a2.pdf}
        \includegraphics[scale=0.24]{plots_a2/scatter_syd_100R_a2.pdf}
        % \includegraphics[scale=0.18]{plots/s1.pdf}
        \caption{Sydney ($256 \times 256$)}
        \label{fig:scatter-sydney}
    \end{subfigure}
    
    
    % DEN
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.24]{plots_a2/scatter_den_50R_a2.pdf}
        \includegraphics[scale=0.24]{plots_a2/scatter_den_100R_a2.pdf}
        % \includegraphics[scale=0.18]{plots/s1.pdf}
        \caption{Den ($257 \times 256$)}
        \label{fig:scatter-den}
    \end{subfigure}
    
    
    
    

    \caption{Computation Time Comparison with Baseline \\ \hspace*{1.3cm} for Various Workspaces 
    % \\ (\textit{X-axis:} $\log{(\text{Runtime(\si{\second})})}$ of (p0h0c0), \textit{Y-axis:} $\log{(\text{Runtime(\si{\second})})}$ 
    \\ \hspace*{1.3cm} (\textit{X-axis:} Runtime(\si{\second}), \textit{Y-axis:} Runtime(\si{\second}))
    \\ \hspace*{1.3cm} (Left: $R = 50$, Right: $R = 100$)  
    }
    \label{fig:scatter_plots}
\end{figure}



==> plots_scatter_b3_adx.tex <==
% SCATTER PLOTS (in split mode) 

\begin{figure*}[!ht]
    
    % RANDOM_200 
    \begin{subfigure}{\linewidth} % Use the subfigure environment
        \centering
        \includegraphics[scale=0.125]{plots_b3/scatter_random_50R_b3_h1m0p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_random_50R_b3_h0m1p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_random_50R_b3_h0m0p1.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_random_50R_b3_h1m1p1.pdf} 
        \hspace*{0.2cm}
        \includegraphics[scale=0.125]{plots_b3/scatter_random_100R_b3_h1m0p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_random_100R_b3_h0m1p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_random_100R_b3_h0m0p1.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_random_100R_b3_h1m1p1.pdf}
        
        \caption{Random ($200 \times 200$)}
        \label{figadx:scatter-random}
    \end{subfigure}

    
    % WAREHOUSE
    \begin{subfigure}{\linewidth} % Use the subfigure environment
        \centering
        \includegraphics[scale=0.125]{plots_b3/scatter_ware_50R_b3_h1m0p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_ware_50R_b3_h0m1p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_ware_50R_b3_h0m0p1.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_ware_50R_b3_h1m1p1.pdf}
        \hspace*{0.2cm}
        \includegraphics[scale=0.125]{plots_b3/scatter_ware_100R_b3_h1m0p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_ware_100R_b3_h0m1p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_ware_100R_b3_h0m0p1.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_ware_100R_b3_h1m1p1.pdf}
        
        \caption{Warehouse ($123 \times 321$)}
        \label{figadx:scatter-warehouse}
    \end{subfigure}
    

    % PARIS
    \begin{subfigure}{\linewidth} % Use the subfigure environment
        \centering
        \includegraphics[scale=0.125]{plots_b3/scatter_paris_50R_b3_h1m0p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_paris_50R_b3_h0m1p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_paris_50R_b3_h0m0p1.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_paris_50R_b3_h1m1p1.pdf}
        \hspace*{0.2cm}
        \includegraphics[scale=0.125]{plots_b3/scatter_paris_100R_b3_h1m0p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_paris_100R_b3_h0m1p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_paris_100R_b3_h0m0p1.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_paris_100R_b3_h1m1p1.pdf}
        
        \caption{Paris ($256 \times 256$)}
        \label{figadx:scatter-paris}
    \end{subfigure}

    
    
    % SYDNEY
    \begin{subfigure}{\linewidth} % Use the subfigure environment
        \centering
        \includegraphics[scale=0.125]{plots_b3/scatter_syd_50R_b3_h1m0p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_syd_50R_b3_h0m1p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_syd_50R_b3_h0m0p1.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_syd_50R_b3_h1m1p1.pdf}
        \hspace*{0.2cm}
        \includegraphics[scale=0.125]{plots_b3/scatter_syd_100R_b3_h1m0p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_syd_100R_b3_h0m1p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_syd_100R_b3_h0m0p1.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_syd_100R_b3_h1m1p1.pdf}
        
        \caption{Sydney ($256 \times 256$)}
        \label{figadx:scatter-sydney}
    \end{subfigure}
    
    
    
    % DEN
    \begin{subfigure}{\linewidth} % Use the subfigure environment
        \centering
        \includegraphics[scale=0.125]{plots_b3/scatter_den_50R_b3_h1m0p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_den_50R_b3_h0m1p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_den_50R_b3_h0m0p1.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_den_50R_b3_h1m1p1.pdf}
        \hspace*{0.2cm}
        \includegraphics[scale=0.125]{plots_b3/scatter_den_100R_b3_h1m0p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_den_100R_b3_h0m1p0.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_den_100R_b3_h0m0p1.pdf}
        \includegraphics[scale=0.125]{plots_b3/scatter_den_100R_b3_h1m1p1.pdf}
        
        \caption{Den ($257 \times 256$)}
        \label{figadx:scatter-den}
    \end{subfigure}
    
    
    
    

    \caption{Computation Time Comparison with Baseline for Various Workspaces 
    % \\ (\textit{X-axis:} $\log{(\text{Runtime(\si{\second})})}$ of (p0h0c0), \textit{Y-axis:} $\log{(\text{Runtime(\si{\second})})}$ 
    \\ \hspace*{1.3cm} (\textit{X-axis:} Runtime(\si{\second}), \textit{Y-axis:} Runtime(\si{\second}))
     \hspace*{1.3cm} (Leftmost four plots: $R = 50$, Rightmost four plots: $R = 100$)  
    }
    \label{figadx:scatter_plots}
\end{figure*}



==> plots_violin.tex <==
% VIOLIN PLOTS

\begin{figure}[!ht]
    % SYDNEY
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.27]{plots/violin_syd_50R.pdf}
        \includegraphics[scale=0.27]{plots/violin_syd_100R.pdf}
        % \includegraphics[scale=0.18]{plots/v1.pdf}
        \caption{Sydney ($256 \times 256$)}
        \label{fig:violin-sydney}
    \end{subfigure}
    
    % WAREHOUSE
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.27]{plots/violin_ware_50R.pdf}
        \includegraphics[scale=0.27]{plots/violin_ware_100R.pdf}
        % \includegraphics[scale=0.18]{plots/v1.pdf}
        \caption{Warehouse ($123 \times 321$)}
        \label{fig:violin-warehouse}
    \end{subfigure}
    
    % DEN
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.27]{plots/violin_den_50R.pdf}
        \includegraphics[scale=0.27]{plots/violin_den_100R.pdf}
        % \includegraphics[scale=0.18]{plots/v1.pdf}
        \caption{Den ($257 \times 256$)}
        \label{fig:violin-den}
    \end{subfigure}
    
    % RANDOM_200
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.27]{plots/violin_random_50R.pdf}
        \includegraphics[scale=0.27]{plots/violin_random_100R.pdf}
        % \includegraphics[scale=0.18]{plots/v1.pdf}
        \caption{Random ($200 \times 200$)}
        \label{fig:violin-random}
    \end{subfigure}
    
    
    

    \caption{Ablation Study using Violin Plots for Different Workspace 
    \\ \hspace*{1.3cm} (\textit{X-axis:} Approaches, \textit{Y-axis:} Runtime(\si{\second})) 
    \\ \hspace*{1.3cm} (Left: $R = 50$, Right: $R = 100$)}
    \label{fig:violin_plots}
\end{figure}


==> plots_violin_a2_adx.tex <==
% VIOLIN PLOTS

\begin{figure}[!ht]
    
    % RANDOM_200
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.27]{plots_a2/violin_random_50R_a2.pdf}
        \includegraphics[scale=0.27]{plots_a2/violin_random_100R_a2.pdf}
        % \includegraphics[scale=0.18]{plots/v1.pdf}
        \caption{Random ($200 \times 200$)}
        \label{figadx:violin-random}
    \end{subfigure}
    
    
    % WAREHOUSE
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.27]{plots_a2/violin_ware_50R_a2.pdf}
        \includegraphics[scale=0.27]{plots_a2/violin_ware_100R_a2.pdf}
        % \includegraphics[scale=0.18]{plots/v1.pdf}
        \caption{Warehouse ($123 \times 321$)}
        \label{figadx:violin-warehouse}
    \end{subfigure}
    
    
    % PARIS
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.27]{plots_a2/violin_paris_50R_a2.pdf}
        \includegraphics[scale=0.27]{plots_a2/violin_paris_100R_a2.pdf}
        % \includegraphics[scale=0.18]{plots/v1.pdf}
        \caption{Paris ($256 \times 256$)}
        \label{figadx:violin-paris}
    \end{subfigure}

    
    % SYDNEY
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.27]{plots_a2/violin_syd_50R_a2.pdf}
        \includegraphics[scale=0.27]{plots_a2/violin_syd_100R_a2.pdf}
        % \includegraphics[scale=0.18]{plots/v1.pdf}
        \caption{Sydney ($256 \times 256$)}
        \label{figadx:violin-sydney}
    \end{subfigure}

    
    % DEN
    \begin{subfigure}{\columnwidth} % Use the subfigure environment
        \includegraphics[scale=0.27]{plots_a2/violin_den_50R_a2.pdf}
        \includegraphics[scale=0.27]{plots_a2/violin_den_100R_a2.pdf}
        % \includegraphics[scale=0.18]{plots/v1.pdf}
        \caption{Den ($257 \times 256$)}
        \label{figadx:violin-den}
    \end{subfigure}
    
    
    
    

    \caption{Ablation Study for Various Workspaces 
    \\ \hspace*{1.3cm} (\textit{X-axis:} Approaches, \textit{Y-axis:} Runtime(\si{\second})) 
    \\ \hspace*{1.3cm} (Left: $R = 50$, Right: $R = 100$)}
    \label{figadx:violin_plots}
\end{figure}


==> table_1.tex <==
% Table 1 v1 : Internal data between p0m0h0 and p1m1h1 

\begin{table*}[!ht]
\centering
\fontsize{9pt}{10pt}\selectfont
% \setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccr}
\toprule
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}WS\\Size\end{tabular}}} &
  \multirow{2}{*}{\textbf{R}} &
    \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Unconst. Path Comp. \end{tabular}}} &
    \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Const. Path Comp.\end{tabular}}} &
    \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Assignment Comp. \end{tabular}}} &
    \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Timeout Count \end{tabular}}} &
     
    \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Speedup\end{tabular}}} \\ \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8}  \cmidrule(r){9-10}
    &
    &
    \textbf{h0m0p0}  &
    \textbf{h1m1p1}  &
    
    \textbf{h0m0p0}  &
    \textbf{h1m1p1}  &

    \textbf{h0m0p0}  &
    \textbf{h1m1p1}  &

    \textbf{h0m0p0}  &
    \textbf{h1m1p1}  &

    
    \\
\midrule


\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Random\\$200$$\times$$200$\end{tabular}} 

& $50$    &  $2500_{\pm 0}$  & $224.79_{\pm 97.18}$  &  $40.88_{\pm 232.86}$  &  $3.71_{\pm 10.08}$  &  $73.73_{\pm 134.66}$  &  $7.42_{\pm 29.53}$  &  $2$  &  $1$   &  $9.69$  \\ 

& $100$  &  $10000_{\pm 0}$   & $708.05_{\pm 244.66}$  &  $479.21_{\pm 1256.32}$  &  $11.26_{\pm 14.08}$  &  $2945.16_{\pm 6873.20}$  &  $124.82_{\pm 279.20}$  &  $12$  &  $9$   &  $5.86$  \\ 


\midrule


\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Warehouse\\$123$$\times$$321$\end{tabular}} 
& $50$   &  $2500_{\pm 0}$  & $212.71_{\pm 83.14}$  &  $15.17_{\pm 45.67}$  &  $3.58_{\pm 3.11}$  &  $115.60_{\pm 244.65}$  &  $12.25_{\pm 34.24}$  &  $1$  &  $2$   &  $11.61$  \\ 

& $100$  &  $10000_{\pm 0}$   & $646.73_{\pm 212.54}$  &  $552.00_{\pm 2004.51}$  &  $320.03_{\pm 1134.85}$  &  $2602.64_{\pm 6216.23}$  &  $192.52_{\pm 250.13}$  &  $14$  &  $15$   &  $2.47$  \\ 


\midrule


\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Sydney\\$256$$\times$$256$\end{tabular}} 
& $50$   &  $2500_{\pm 0}$   \\ 

& $100$  &  $10000_{\pm 0}$      \\ 


\midrule


\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Den\\$257$$\times$$256$\end{tabular}} 
& $50$   &  $2500_{\pm 0}$  & $422.22_{\pm 129.26}$  &  $7.19_{\pm 14.91}$  &  $2.81_{\pm 2.86}$  &  $69.66_{\pm 73.77}$  &  $1.06_{\pm 0.35}$  &  $13$  &  $14$   &  $1.52$  \\ 


& $100$  &  $10000_{\pm 0}$  & $1266.28_{\pm 523.91}$  &  $264.56_{\pm 404.94}$  &  $12.22_{\pm 15.35}$  &  $752.33_{\pm 532.86}$  &  $1.56_{\pm 1.30}$  &  $31$  &  $21$   &  $7.73$  \\  



\bottomrule
\end{tabular}
}
\caption{ Additional Performance Comparison of Baseline ($\mathtt{h0m0p0}$) vs. Our Approach ($\mathtt{h1m1p1}$)   }
\label{table:table_1}
\end{table*}




==> ztable1-backup.tex <==
% Table 1 v1 : Internal data between p0m0h0 and p1m1h1 

\begin{table*}[!ht]
\centering
\fontsize{9pt}{9pt}\selectfont
% \setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccr}
\toprule
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}WS\\Size\end{tabular}}} &
  \multirow{2}{*}{\textbf{R}} &
    \multicolumn{2}{c}{\textbf{ Uncon. Path Comp. Savings }} &
    \multicolumn{2}{c}{\textbf{ Path Memo. Savings }} &
    \multicolumn{2}{c}{\textbf{ Asgn. Comp. Savings }} &
    % \multicolumn{2}{c}{\textbf{ Total Cost }} &
    
    
    \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Overall\\Speedup\end{tabular}}} \\ \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
    &
    &
    \textbf{h0m0p0}  &
    \textbf{h1m1p1}  &
    
    \textbf{h0m0p0}  &
    \textbf{h1m1p1}  &

    \textbf{h0m0p0}  &
    \textbf{h1m1p1}  &

    % \textbf{Before PP}  &
    % \textbf{After PP}  &
    
      \\
\midrule



\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Sydney\\$256$$\times$$256$\end{tabular}} 
& $50$  & $73.14_{\pm 9.31}$   &   $73.24_{\pm 9.28}$   &   $\hphantom{0}3.66_{\pm 0.83}$   &  $9.10_{\pm 3.16}$      &  $0.05_{\pm 0.01}$  &  \hphantom{0}$3.71_{\pm 0.82}$       &  $2.47$    \\ 

& $100$  & $50.34_{\pm 6.31}$ & $50.58_{\pm 6.59}$ &   $\hphantom{0}6.80_{\pm 1.45}$   &  $39.29_{\pm 18.88}$    &  $0.16_{\pm 0.03}$  &  \hphantom{0}$6.96_{\pm 1.45}$      &  $5.67$    \\ 

% & $400$  & $43.78_{\pm 6.82}$ & $44.16_{\pm 6.98}$ &   $16.77_{\pm 3.58}$  &  $446.55_{\pm 336.09}$  &  $0.44_{\pm 0.07}$  &  $17.21_{\pm 3.58}$   &  $446.99_{\pm 336.64}$ &  $25.97$   \\ 


\midrule


\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Warehouse\\$123$$\times$$321$\end{tabular}} 
& $50$  & $64.54_{\pm 14.51}$ & $64.54_{\pm 14.51}$ &  $\hphantom{0}1.91_{\pm 0.55}$   &  $7.20_{\pm 3.93}$     &  $0.05_{\pm 0.01}$  &  \hphantom{0}$1.96_{\pm 0.55}$  &      $3.70$  \\

& $100$  & $50.10_{\pm 13.44}$ & $50.10_{\pm 13.44}$ &  $\hphantom{0}3.85_{\pm 0.89}$   &  $39.71_{\pm 18.49}$   & $0.16_{\pm 0.06}$   &  \hphantom{0}$4.01_{\pm 0.89}$   &     $9.94$  \\

% & $400$  & $39.32_{\pm 8.52\hphantom{0}}$ & $39.70_{\pm 8.89\hphantom{0}}$ &  $16.82_{\pm 5.82}$  &  $720.37_{\pm 465.80}$  & $0.41_{\pm 0.11}$  &  $17.23_{\pm 5.82}$   & $720.78_{\pm 466.72}$ &    $41.83$  \\

\midrule


\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Den\\$257$$\times$$256$\end{tabular}} 
& $50$  & $74.74_{\pm 13.57}$ & $75.08_{\pm 13.56}$ &  $\hphantom{0}6.10_{\pm 2.06}$    &  $12.95_{\pm 4.18\hphantom{0}}$      &  $0.06_{\pm 0.02}$  &  \hphantom{0}$6.16_{\pm 2.06}$  &    $2.11$  \\ 

& $100$  & $60.62_{\pm 13.84}$ & $61.02_{\pm 14.08}$ &  $10.04_{\pm 4.50}$   &  $68.55_{\pm 49.01}$     &  $0.16_{\pm 0.06}$  &  $10.20_{\pm 4.50}$  &   $6.74$  \\ 

% & $400$  & $47.56_{\pm 7.95\hphantom{0}}$ & $48.80_{\pm 8.64\hphantom{0}}$ &  $25.19_{\pm 6.94}$   &  $750.02_{\pm 439.98}$   &  $0.48_{\pm 0.13}$  &  $25.67_{\pm 6.94}$  & $750.50_{\pm 441.02}$  &  $29.24$ \\ 


\midrule


\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Random\\$200$$\times$$200$\end{tabular}} 
& $50$   & $50.74_{\pm 10.25}$ & $51.14_{\pm 10.31}$ &  $\hphantom{0}3.44_{\pm 0.48}$   &  $7.66_{\pm 1.63}$      & $0.04_{\pm 0.01}$  &  \hphantom{0}$3.48_{\pm 0.48}$  &     $2.21$  \\ 

& $100$   & $41.22_{\pm 7.90\hphantom{0}}$ & $42.48_{\pm 8.09\hphantom{0}}$ &   \hphantom{0}$7.21_{\pm 1.58}$  &  $59.75_{\pm 27.90}$    & $0.10_{\pm 0.02}$  &  \hphantom{0}$7.31_{\pm 1.58}$  &   $8.19$ \\ 

% & $400$   & $34.76_{\pm 5.43\hphantom{0}}$ & $38.86_{\pm 6.90\hphantom{0}}$ & $25.65_{\pm 6.80}$  &  $559.56_{\pm 216.52}$  & $0.27_{\pm 0.05}$  &  $25.92_{\pm 6.81}$  &  $559.83_{\pm 216.86}$  &  $21.60$ \\ 



\bottomrule
\end{tabular}
}
\caption{ Additional Performance Comparison of Baseline ($h0m0p0$) vs. Our Approach ($h1m1p1$) }
\label{table:table_1}
\end{table*}



